Learning to Segment via Cut-and-Paste

This paper presents a weakly-supervised approach to object instance segmentation. Starting with known or predicted object bounding boxes, we learn object masks by playing a game of cut-and-paste in an adversarial learning setup. A mask generator takes a detection box and Faster R-CNN features, and constructs a segmentation mask that is used to cut-and-paste the object into a new image location. The discriminator tries to distinguish between real objects, and those cut and pasted via the generator, giving a learning signal that leads to improved object masks. We verify our method experimentally using Cityscapes, COCO, and aerial image datasets, learning to segment objects without ever having seen a mask in training. Our method exceeds the performance of existing weakly supervised methods, without requiring hand-tuned segment proposals, and reaches 90% of supervised performance.

==> aerial_occluded_houses_figure.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{ c@{\hspace{0.003\textwidth}}c@{\hspace{0.003\textwidth}}c@{\hspace{0.003\textwidth}}c@{\hspace{0.003\textwidth}}c@{\hspace{0.003\textwidth}}c@{\hspace{0.003\textwidth}}c@{\hspace{0.003\textwidth}}c@{\hspace{0.003\textwidth}}c@{\hspace{0.003\textwidth}}c }

\includegraphics[width=1.4cm,height=1.4cm]{Figures/Aerial/Occluded/0499800_37_hires_patch.png} &
\includegraphics[width=1.4cm,height=1.4cm]{Figures/Aerial/Occluded/0499800_1615_hires_patch.png} &
\includegraphics[width=1.4cm,height=1.4cm]{Figures/Aerial/Occluded/0499800_531_hires_patch.png} &
\includegraphics[width=1.4cm,height=1.4cm]{Figures/Aerial/Occluded/0499800_104_hires_patch.png} &
\includegraphics[width=1.4cm,height=1.4cm]{Figures/Aerial/Occluded/0499800_177_hires_patch.png} &
\includegraphics[width=1.4cm,height=1.4cm]{Figures/Aerial/Occluded/0499800_401_hires_patch.png} &
\includegraphics[width=1.4cm,height=1.4cm]{Figures/Aerial/Occluded/0499800_1496_hires_patch.png} &
\includegraphics[width=1.4cm,height=1.4cm]{Figures/Aerial/Occluded/0499800_95_hires_patch.png} \\
% \includegraphics[width=1.4cm,height=1.4cm]{Figures/Aerial/Occluded/0499800_1640_hires_patch.png} &
% \includegraphics[width=1.4cm,height=1.4cm]{Figures/Aerial/Occluded/0499800_94_hires_patch.png} \\

\end{tabular}
\caption{\textbf{Examples of heavily occluded houses.} Houses from aerial imagery tend to have different level of occlusions by nearby trees, the main difference with respect to other datasets is that a random paste position has a high probability of containing plausible occluders (in the form of trees of other greenery). Thus promoting the generator to learn to cut and paste parts of houses. See Figure \ref{figure:aerial_overlays} for aerial imagery examples.}
\label{figure:aerial_occluded}
\end{figure}

==> background.tex <==
\jon{do we need this section?}

==> copy_paste_algorithm.tex <==
\begin{algorithm}[H]
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
 \Input{
 \begin{itemize}
    \item I: input image.
    \item $B_{obj}$: object bounding box of size $W \times H$.
    \item $M\in[0,1]^{m\times m}$: mask of size $m\times m$.
    \item $B_{target}$: target bounding box of size $W \times H$.
    \item p: how much to pad the pasted object (in pixels).
 \end{itemize}
 }
 
 \Output{P: Object pasted onto the background at target location.}
 \BlankLine
 \Begin{
$pad\_ratio \leftarrow p/m$

$\sigma_x \leftarrow 0.5\cdot \frac{W}{m+p}$

$\sigma_y \leftarrow 0.5\cdot \frac{H}{m+p}$

$I_{blurred} \leftarrow gaussian\_blur(I,\sigma_x, \sigma_y)$

$B_{obj\_exp} \leftarrow expand\_box(B_{obj}, pad\_ratio)$

$B_{target\_exp} \leftarrow expand\_box(B_{target}, pad\_ratio)$

$C_{obj} \leftarrow crop\_image(I_{blurred}, B_{obj\_exp})$

$C_{target} \leftarrow crop\_image(I_{blurred}, B_{target\_exp})$

$C_{obj} \leftarrow imresize(C_{obj}, m+p,m+p)$

$C_{target} \leftarrow imresize(C_{target}, m+p,m+p)$

$M_{pad} \leftarrow zero\_pad(M, p)$

$P \leftarrow M_{pad} \cdot C_{obj} + (1-M_{pad}) \cdot C_{target}$ 
}
 
 \caption{Cutting and Pasting objects}
 \label{algorithm:cut-paste}
\end{algorithm}

==> copy_paste_artifacts_figure.tex <==
\begin{figure}[tb]
\centering
\begin{tabular}{ c c c c c }

        \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/42_image_fullres.png} &
        \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/42_bg_fullres.png} &
        \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/42_paste_lowres_area.png} &
        \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/42_paste_lowres_area_bg_nn_obj.png} &
        \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/42_paste_hires.png} \\
        
        (a) & (b) & (c) & (d) & (e) \\
        
\end{tabular}
\caption{\textbf{Illustration of different cut and paste methodologies.} 
%\mbnote{Some tests that would make sense: 1) Baseline correct sampling, 2) Aliasing Test: No blurring of pasted image before sampling , 3) Blurring test: Mask is lower res than src/dst images}
%
There are multiple options for how to copy and paste objects assuming the mask is at a lower resolution than the full resolution object. (a) and (b) are the original high resolution object and target background; (c) result of cutting and pasting at the resolution of the mask after downsampling the images; (d) incorrect downsampling of the object without antialiasing; (e) cut and paste at the full resolution using a bi-cubic upsampled mask. Notice the aliasing artifacts on the pants of the person in image(d) and the halo artifacts of the mask upsampling in image (e), both are easily noticeable.
}
\label{figure:copy_paste_artifacts}
\end{figure}



% \begin{figure}
% \centering
% \begin{tabular}{ c c c c c }

%         \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/1_image_fullres.png} &
%         \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/1_bg_fullres.png} &
%         \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/1_paste_lowres_nn.png} &
%         \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/1_paste_lowres_smooth.png} &
%         \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/1_paste_lowres_smooth_mid.png} \\
        
%         \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/2_image_fullres.png} &
%         \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/2_bg_fullres.png} &
%         \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/2_paste_lowres_nn.png} &
%         \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/2_paste_lowres_smooth.png} &
%         \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/2_paste_lowres_smooth_mid.png} \\

%         (a) & (b) & (c) & (d) & (e) \\
        
% \end{tabular}
% \caption{\textbf{Comparison of different copy and paste methods.} \mbnote{Some tests that would make sense: 1) Baseline correct sampling, 2) Aliasing Test: No blurring of pasted image before sampling , 3) Blurring test: Mask is lower res than src/dst images}
% %
% There are multiple options for how to copy and paste objects depending on image and mask re-sampling. (a) and (b) are the original high resolution object and target background; The result of copy pasting at a lower resolution that is equal to the mask resolution while downsampling the images with (d) and without (c) an anti-aliasing filter; (e) show the effect of copy pasting at a resolution higher than the mask's, in which case the mask must be upsampled to the correct size.
% %
% Our experiments showed using an anti-aliasing filter reduces visible artifact at the borders on objects. We also saw that trying to copy paste at a resolution that is higher than the predicted mask (as can be seen in(e)) results in blurring of the mask and halo artifacts around objects. Both types of artifacts were easily detectable by the discriminator and reduced mask pixel accuracy by as much as 
% }
% \label{figure:copy_paste_artifacts}
% \end{figure}

%\begin{figure}
%\centering
%\scriptsize
%\centering
%\begin{tabular}{ c c c c c }
%        Object & Background & c.p. high res & c.p. low res  & c.p. low res + blur \\
%        \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/2_image_fullres.png} &
%        \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/2_bg_fullres.png} &
%        \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/2_paste_hires.png} &
%        \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/2_paste_lowres.png} &
%        \includegraphics[width=2.2cm,height=3.2cm]{Figures/CopyPasteArtifacts/2_paste_lowres_smooth.png} \\
%        
%\end{tabular}
%\caption{\textbf{Comparison of different copy and paste options.} \mbnote{Some tests that would make sense: 1) Baseline correct sampling, 2) Aliasing Test: No blurring of pasted image before sampling , 3) Blurring test: Mask is lower res than src/dst images} From left to right: the original high resolution bounding box containing an object, a bounding box containing a high resolution background, the result of copy pasting the object onto the background using an upsampled mask, the result of copy pasting the object at a lower resolution without and with blurring. \tal{Maybe we should add zoom-in areas so we can see the artifacts better.}}
%\label{figure:copy_paste_artifacts}
%\end{figure}

==> limitations.tex <==
%Some of our method's limitation are due to its limited ability to handle data which includes very crowded images leaving no place to paste objects into, or data in which objects are very occluded making it hard to paste them in locations that will have a believable occluder, or objects that appear on uniform background (such as kites or planes). In addition some objects have a very strong semantic connection to other objects making it hard to separate them without better placement techniques for the pasted objects (for instance eye-glasses, hats or shirts which almost always appear on a person). Another limitation is the requirement of having a very large dataset, in COCO most classes have about 10K instances compared to more that 100K in Cityscapes. 

%We think that future work should research how to incorporate the positioning of fake objects into the learning process. While being an interesting topic on its own we believe this might also improve segmentation performance.

% \jon{how do people feel if we just made this the conclusion section?}

% \begin{itemize}
%     \item pasting is problematic if images are crowded (as in COCO)
%     \item some objects can only be placed in very specific positions due to strong semantic connections such as hats, shirts and bikes.
%     \item Masks aren't as fine as the ones produced by supervised training at this point.
%     \item In some sense, things are never perfectly independent of their surroundings — in this paper we used heuristics for object placement, but future work might directly tackle this problem of placement.
%     \item occlusions
%     \item Large amounts of data are needed (even some COCO classes dont have enough images/instances) we should explain that the discriminator overfits to the real examples when the data is small < ~10000 instances.
    
% \end{itemize}


